Heavy Quark Mass Effects in Deep Inelastic Scattering and Global QCD Analysis

A new implementation of the general PQCD formalism of Collins, including heavy quark mass effects, is described. Important features that contribute to the accuracy and efficiency of the calculation of both neutral current (NC) and charged current (CC) processess are explicitly discussed. This new implementation is applied to the global analysis of the full HERA I data sets on NC and CC cross sections, with correlated systematic errors, in conjunction with the usual fixed-target and hadron collider data sets. By using a variety of parametrizations to explore the parton parameter space, robust new parton distribution function (PDF) sets (CTEQ6.5) are obtained. The new quark distributions are consistently higher in the region x ~ 10^{-3} than previous ones, with important implications on hadron collider phenomenology, especially at the LHC. The uncertainties of the parton distributions are reassessed and are compared to the previous ones. A new set of CTEQ6.5 eigenvector PDFs that encapsulates these uncertainties is also presented.

==> text/HQmDis.pre.tex <==
\newcommand{\DATE}  {\today}

\newcommand{\PPrtNo}
{
MSU-HEP-0605
}
\newcommand{\TITLE}
{ Heavy Quark Mass Effects in Deep Inelastic Scattering and Global
QCD Analysis
}
\newcommand{\THANKS}
{

}
\newcommand{\AUTHORS}
{W.K.~Tung$^{a,b}$, H.L.~Lai$^c$, A.~Belyaev$^a$, J.~Pumplin$^a$,
D.~Stump$^a$, and C.-P.~Yuan$^a$}
\newcommand{\INST}
{
$^a$ Michigan State University, E. Lansing, MI, USA \\
$^b$ University of Washington, Seattle, WA, USA \\
$^c$ Taipei Municipal University of Education, Taipei, Taiwan
}
\newcommand{\ABSTRACT}
{A new implementation of the general PQCD formalism of Collins, including
heavy quark mass effects, is described. Important features that contribute to
the accuracy and efficiency of the calculation of both neutral current (NC)
and charged current (CC) processess are explicitly discussed. This new
implementation is applied to the global analysis of the full HERA I data sets
on NC and CC cross sections, with correlated systematic errors, in
conjunction with the usual fixed-target and hadron collider data sets. By
using a variety of parametrizations to explore the parton parameter space,
robust new parton distribution function (PDF) sets (CTEQ6.5) are obtained.
The new quark distributions are consistently higher in the region
$x\sim10^{-3}$ than previous ones, with important implications on hadron
collider phenomenology, especially at the LHC. The uncertainties of the
parton distributions are reassessed and are compared to the previous ones. A
new set of CTEQ6.5 eigenvector PDFs that encapsulates these uncertainties is
also presented.}
					% page format of the logical page
\textwidth  = 6.5 in
\textheight = 9.0 in

\topmargin     = 1.0 in
\oddsidemargin = 1.0 in
					% printer device-dependent offsets
\voffset = -1.60 in
\hoffset = -1.00 in

\setlength{\parindent}{2 em}
\setlength{\itemindent}{0 em}
\renewcommand{\baselinestretch}{1.1}

%\newcommand{\}[]{}
\newcommand{\msbar}{\mbox{\small {$\overline {MS}$}}}


==> text/front.tex <==
% Standard Simple Cover Page for Papers -- wkt 1/11/95

\begin{titlepage}

\noindent
\begin{tabular}{l} \DATE
\end{tabular}
\hfill
\begin{tabular}{l}
\PPrtNo
\end{tabular}

\vspace{1cm}

\begin{center}
                           % Title
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
{
\LARGE \TITLE
%\footnote[2]{\THANKS}
}

\vspace{1.25cm}
                          % Authors
{\large  \AUTHORS}

\vspace{1.25cm}

                          % Institutions
\INST
\end{center}

\vfill

\ABSTRACT                 % Abstract

\vfill

\newpage
\end{titlepage}

%\renewcommand{\thefootnote}{\arabic{footnote}}   % Has to be outside titlepage
%\setcounter{footnote}{0}

